An Immersed Boundary Hierarchical B-spline method for flexoelectricity

This paper develops a computational framework with unfitted meshes to solve linear piezoelectricity and flexoelectricity electromechanical boundary value problems including strain gradient elasticity at infinitesimal strains. The high-order nature of the coupled PDE system is addressed by a sufficiently smooth hierarchical B-spline approximation on a background Cartesian mesh. The domain of interest is embedded into the background mesh and discretized in an unfitted fashion. The immersed boundary approach allows us to use B-splines on arbitrary domain shapes, regardless of their geometrical complexity, and could be directly extended, for instance, to shape and topology optimization. The domain boundary is represented by NURBS, and exactly integrated by means of the NEFEM mapping. Local adaptivity is achieved by hierarchical refinement of B-spline basis, which are efficiently evaluated and integrated thanks to their piecewise polynomial definition. Nitsche's formulation is derived to weakly enforce essential boundary conditions, accounting also for the non-local conditions on the non-smooth portions of the domain boundary (i.e. edges in 3D or corners in 2D) arising from Mindlin's strain gradient elasticity theory. Boundary conditions modeling sensing electrodes are formulated and enforced following the same approach. Optimal error convergence rates are reported using high-order B-spline approximations. The method is verified against available analytical solutions and well-known benchmarks from the literature.

==> Images/Sec_02/02_Potential.tex <==
\section{Variational formulation and associated boundary value problem}\label{sec_02}
%%%%%
\subsection{Notation and preliminary definitions}
%%%%%
Let $\Omega$ be a physical domain in $\mathbb{R}^3$
%, as depicted in figure \ref{fig_2_1_1}
. The domain boundary, $\partial\Omega$, can be conformed by several smooth portions as $\partial\Omega=\bigcup_f\partial\Omega_f$ (\fig\ref{fig_2_1_2}).
At each point $\x\in\partial\Omega_f$ we define $\n^f$ as the outward unit \emph{normal vector}.
The boundary of the $f$-th portion of $\partial\Omega$ is denoted as $\partial\partial\Omega_f$, which is a closed curve. At each point $\x\in \partial\partial\Omega_f$ we define $\m^f$ as the unit \emph{co-normal vector} pointing outwards of $\partial\Omega_f$, which is orthogonal to the normal vector $\n^f$ and to the tangent vector of the curve $\partial\partial\Omega_f$, $\tv^f$ (see \fig\ref{fig_2_1_3} and \ref{fig_2_1_4}). The orientation of $\tv^f$ is arbitrary and not relevant in the derivations next.

\begin{figure}[b]\centering
%	\begin{subfigure}[t]{.17\textwidth}\centering
%		\captionof{figure}{}
%		\includegraphics[scale=0.17]{Images/Sec_02/1c2.pdf}
%		\vfill\label{fig_2_1_1}
%	\end{subfigure}%
	\begin{subfigure}[t]{.34\textwidth}\centering
		\captionof{figure}{}
		\includegraphics[scale=0.17]{Images/Sec_02/2c2_good.pdf}
		\vfill\label{fig_2_1_2}
	\end{subfigure}%
	\begin{subfigure}[t]{.25\textwidth}\centering
		\captionof{figure}{}
		\includegraphics[scale=0.17]{Images/Sec_02/3c2_good.pdf}
		\vfill\label{fig_2_1_3}
	\end{subfigure}%
	\begin{subfigure}[t]{.24\textwidth}\centering
		\captionof{figure}{}
		\includegraphics[scale=0.17]{Images/Sec_02/4c2_good.pdf}
		\vfill\label{fig_2_1_4}
	\end{subfigure}
	\caption{Sketch of the geometry of $\Omega\in\mathbb{R}^3$.
		%a) Physical domain $\Omega\in\mathbb{R}^3$, b) 
		\emph{a)} Detail of $\partial\Omega$ subdivided in smooth portions $\partial\Omega_i$ and $\partial\Omega_j$, with their corresponding normal vectors $\n^i$ and $\n^j$, \emph{b)} detail of $\partial\Omega_i$, with the triplet $\{\m^i,\tv^i,\n^i\}$ defined on $\partial\partial\Omega_i$, and \emph{c)} detail of $\partial\Omega_j$, with the triplet $\{\m^j,\tv^j,\n^j\}$ defined on $\partial\partial\Omega_j$.}
	\label{fig_2_1}
\end{figure}

The operators that appear throughout this Section are defined next.
The \emph{spatial derivative} of a function $f$ with respect to the coordinate $x_i$ is denoted by $\partial_i$ or the subindex $i$ after a comma, that is, $\frac{\partial}{\partial x_i}(f)=\partial_if=f_{,i}$.
The \emph{gradient} operator is denoted as $\gradient(~~)$, and the \emph{divergence} operator as $\divergence(~~)$. For instance, for a second order tensor $\toMat{A}$, they are defined as $[\gradient(\toMat{A})]_{ijk}\coloneqq\partial_kA_{ij}=A_{ij,k}$, and $[\divergence(\toMat{A})]_i\coloneqq\partial_jA_{ij}=A_{ij,j}$, respectively.\\
The \emph{symmetrized gradient} $\symmetricGradient{(~~)}$ of a vector field $\toVect{a}$ is defined as:
\begin{equation}
\left[\symmetricGradient{(\toVect{a})}\right]_{ij}\coloneqq\frac{1}{2}\left[\gradient{(\toVect{a})}+\gradient{(\toVect{a})}^T\right]_{ij}=\frac{1}{2}(a_{i,j}+a_{j,i}).
\end{equation}
On the domain boundary $\partial\Omega$ the derivative in the normal direction, namely the \emph{normal derivate}, is denoted by $\partial^n$. For instance, the normal derivative of a vector field $\toVect{a}$ is defined as $\partial^n(\toVect{a})\coloneqq\gradient(\toVect{a})\cdot\n$.
The gradient and divergence operators can be decomposed on $\partial\Omega$ into their normal and tangential components as $\gradient(~~)=\partial^n(~~)\n+\surfaceGradient(~~)$ and $\divergence(~~)=\partial^n(~~)\cdot\n+\surfaceDivergence(~~)$, respectively,
where $\surfaceGradient(~~)$ and $\surfaceDivergence(~~)$ denote the \emph{surface gradient}  and \emph{surface divergence} operators, namely the projection of the gradient and divergence operators onto the tangent space of $\partial\Omega$.
For a second order tensor $\toMat{A}$ they are expressed as
\begin{subequations}\begin{align}
\left[\surfaceGradient(\toMat{A})\right]_{ijk}=\surfaceGradient_kA_{ij}\coloneqq&
%\left[\gradient{(\toMat{A})}\cdot\Projector\right]_{ijk}=
A_{ij,l}P_{lk},\\
\left[\surfaceDivergence(\toMat{A})\right]_i=\surfaceGradient_jA_{ij}\coloneqq&
%\left[\gradient{(\toMat{A})}:\Projector\right]_i=
A_{ij,k}P_{jk},
\end{align}\end{subequations}
respectively, where $\Projector$ is the \emph{projection operator} defined on $\partial\Omega$ as 
$\left[\Projector\right]_{ij}\coloneqq%\toMat{I}-\n\otimes\n=
\delta_{ij}-n_in_j$, being $\delta_{ij}$ the Kronecker delta.

The formulation involves second-order measures of the geometry, namely curvatures of $\partial\Omega$. The tensor that contains this information is known as the \emph{shape operator} $\ShapeOperator$ (also known as curvature tensor) \cite{Block1997}, defined on the surface $\partial\Omega$ as
\begin{equation}
[\ShapeOperator]_{ij}\coloneqq-\left[\surfaceGradient(\n)\right]_{ij}=-n_{i,l}P_{lj}.
\end{equation}
The \emph{mean curvature} $H$ of a surface is an invariant, expressed in terms of $\ShapeOperator$ as
\begin{equation}
H\coloneqq\frac{1}{2}\trace{\ShapeOperator}=-\frac{1}{2}\surfaceDivergence\n=-\frac{1}{2}n_{i,j}P_{ij}.
\end{equation}
With $\ShapeOperator$ and $H$ we define a tensor which arises in the formulation 
(see \ref{sec_app01}), that we name \emph{second-order geometry tensor} $\CurvatureProjector$ and is defined as:
\begin{equation}
\left[\CurvatureProjector\right]_{ij}\coloneqq S_{ij}-2Hn_in_j.
\end{equation}
On the curve $C^{ij}\coloneqq\partial\partial\Omega_i\cap\partial\partial\Omega_j$, $(i\neq j)$ we define the \emph{jump} operator $\jump{~~}$ acting on a given quantity $\toVect{a}$ as the sum of that quantity evaluated at both sides of the curve, namely
$\jump{\toVect{a}}\coloneqq\toVect{a}^i+\toVect{a}^j$, where $\toVect{a}^k$ is the value of $\toVect{a}$ from $\partial\Omega_k$ (see \fig\ref{fig_2_1_2}).
Note that a \emph{sum} is considered in the definition of the jump, so that $\jump{\m\times\n}$ vanishes in the case $C^{ij}$ is defined along a smooth region of $\partial\Omega$,
where $\m^i=-\m^j$ and $\n^i=\n^j$.

Finally, we denote the \emph{first variation} of a certain functional $F[f_1,\dots,f_n]$ with respect to the function $f_i$ as the functional
\begin{equation}
\var[f_i]{F}[f_1,\dots,f_n;\psi_i]
\coloneqq
\frac{d}{d\epsilon}F[f_1,\dots,f_{i-1},f_i+\epsilon\psi_i,f_{i+1},\dots,f_n]\Big{|}_{\epsilon=0},
\end{equation}
where $\epsilon\in\mathbb{R}$, and the function $\psi_i$ is the variation of $f_i$ (hence denoted also as ${\delta\!f}_i$), defined on the same functional space as $f_i$. The variation of $F[f_1,\dots,f_n]$ with respect to all the functions $f_1,\dots,f_n$ is denoted as
\begin{equation}
\var{F}[f_1,\dots,f_n;\psi_1,\dots,\psi_n]
\coloneqq\sum_{i=1}^n \var[f_i]{F}[f_1,\dots,f_n;\psi_i].
\end{equation}
The \emph{second variation} of $F[f_1,\dots,f_n]$ with respect to the function $f_i$ in the direction $\psi_i$ is denoted by $\vvar[f_i]{F}[f_1,\dots,f_n;\psi_i]$, and is defined as the first variation of the functional $\var[f_i]{F}[f_1,\dots,f_n;\psi_i]$ with respect to $f_i$, \ie
\begin{equation}
\vvar[f_i]{F}[f_1,\dots,f_n;\psi_i]
\coloneqq
\var[f_i]{\Big(\var[f_i]{F}[f_1,\dots,f_n;\psi_i]\Big)}[f_1,\dots,f_n;\psi_i],
\end{equation}
where $\psi_i$ is the variation of the function $f_i$ for both variations of $F$.
%%%
\subsection{Standard variational formulation}
%%%
A continuum model for flexoelectric materials can be obtained by coupling a strain-gradient elasticity model with classical electrostatics, through the piezoelectric and flexoelectric effects.
The state variables are the displacement field $\Displacement$ and the electric potential $\phi$.
The strain tensor and the electric field are given by 
\begin{equation}
[\Strain(\Displacement)]_{ij}=[\Strain(\Displacement)]_{ji}\coloneqq\left[\symmetricGradient(\Displacement)\right]_{ij}=\frac{1}{2}(u_{i,j}+u_{j,i}),\label{eq_str}
\end{equation}
\begin{equation}
[\E(\phi)]_l\coloneqq-[\gradient\phi]_l=-\phi_{,l}.
\end{equation}
The bulk energy density $\mathcal{H}^\Omega$ in a flexoelectric material can be stated as \cite{Mao2014,Abdollahi2014, Abdollahi2015a, Abdollahi2015b}
\begin{equation}\label{eq_FlexRawEnergy}
\mathcal{H}^\Omega[\Displacement,\phi]=\mathcal{H}^\Omega[\Strain,\gradient\Strain,\E]\coloneqq\frac{1}{2}\strain_{ij}\elast_{ijkl}\strain_{kl}+\frac{1}{2}\strain_{ij,k}\strGr_{ijklmn}\strain_{lm,n}-\frac{1}{2}E_{l}\dielec_{lm}E_{m}-E_{l}\piezo_{lij}\strain_{ij}-E_{l}\flexo_{lijk}\strain_{ij,k}.
\end{equation}
The first two terms correspond to the mechanical energy density of a strain-gradient elastic material, in the Form II of the original paper of Mindlin \cite{Mindlin1964} about strain gradient elasticity. The tensor $\elast_{ijkl}=\elast_{klij}=\elast_{jikl}=\elast_{ijlk}$ is the fourth-order \emph{elasticity tensor} and $\strGr_{ijklmn}=\strGr_{lmnijk}=\strGr_{jiklmn}=\strGr_{ijkmln}$ is the sixth-order \emph{strain-gradient elasticity tensor}.
The third term is the electrostatic energy density, where $\dielec_{lm}=\dielec_{ml}$ is the second-order \emph{dielectricity tensor}. The last two terms correspond to the piezoelectric and flexoelectric effects, where $\piezo_{lij}=\piezo_{lji}$ is the third-order \emph{piezoelectric tensor} and $\flexo_{lijk}=\flexo_{ljik}$ the fourth-order \emph{flexoelectric tensor}.

Alternative descriptions could also be considered, writing the bulk energy density in terms of other quantities instead of the electric field $\E$, such as the polarization $\toVect{p}$ or the electric displacement $\ElectricDisp=\varepsilon_0\E+\toVect{p}$, where $\varepsilon_0$ is the vacuum permittivity constant. As argued in \cite{Liu2014}, all of them are valid, but the choice of $\E$ facilitates the derivation of equilibrium equations, which are simpler than those in terms of $\toVect{p}$, allowing for simpler numerical methods for solving the associated boundary value problems.
Some authors \cite{Shen2010,Sharma2010,Majdoub2008,Majdoub2009} describe the energy density as $\mathcal{H}^\Omega[\Strain,\gradient\Strain,\toVect{p},\gradient\toVect{p}]$ accounting for the \emph{polarization gradient} theory instead of strain gradient elasticity. We consider the simplified model in \eq\eqref{eq_FlexRawEnergy} since \emph{i)} the quadratic term to the electric field gradient is assumed to be negligible for the problems we are interested in, and \emph{ii)} the last term in \eq\eqref{eq_FlexRawEnergy} describes both the \emph{direct} and \emph{converse} flexoelectric effects as a Lifshitz invariant (see \cite{Landau2013,Sharma2010,Abdollahi2014} for details), leading to the same equilibrium equations as if both terms were treated separately.
%For a different set of flexoelectric problems, such as in ferroelectric domain wall simulations \cite{}, the polarization field is likely to undergo large gradients, and therefore the bulk energy density is conveniently defined as $\mathcal{H}^\Omega[\Strain,\toVect{p},\gradient\toVect{p}]$, where polarization gradient is incorporated instead of strain gradient elasticity.
We also note that either non-local mechanical or electrical effects (or both) must be introduced in the flexoelectric problem in order to get a meaningful energy density from a physical point of view, but also to get numerically stable formulations. It's worth noting that incorporating the polarization gradient theory to the present formulation is straightforward by following the same derivations highlighted in the present paper.

The contribution from external loads is presented next. Being $\toVect{b}$ the \emph{body force} per unit volume, and $q$ the \emph{free charge} per unit volume, their work per unit volume is
\begin{equation}\label{eq_ExternalBulk}
\mathcal{W}^{\Omega}[\Displacement,\phi]\coloneqq -b_iu_i+q\phi.
\end{equation}

Additional external loads are present on the domain boundary. In a strain gradient elasticity formulation \cite{Mindlin1964}, those are the \emph{traction} $\Traction$ and the \emph{double traction} $\HighOrderTraction$, which are the conjugates of the displacement $\Displacement$ and the normal derivative of the displacement $\partial^n(\Displacement)$ on $\partial\Omega$, respectively. The electrical boundary load is the \emph{surface charge density} $w$, which is conjugate of the electric potential $\phi$ on $\partial\Omega$. The work of the external loads per unit area is
\begin{equation}\label{eq_ExternalBoundary}
\mathcal{W}_0^{\partial\Omega}[\Displacement,\phi]\coloneqq -t_iu_i-r_i\partial^nu_i+w\phi.
\end{equation}

Moreover, as dictated by strain gradient elasticity theory \cite{Mindlin1964}, an additional \emph{force per unit length} $\HighOrderJump$ arises at the edges $C$ of the boundary, \ie at the union of the edges formed by the intersection of the portions of the boundary, in case $\partial\Omega$ is not smooth (see \fig\ref{fig_2_1_2}). That is, at $C=\bigcup_f\partial\partial\Omega_f$. The force $\HighOrderJump$ is the conjugate of the displacement $\Displacement$ on $C$. Hence, its work per unit length is
\begin{equation}\label{eq_ExternalLine}
\mathcal{W}_0^C[\Displacement,\phi]\coloneqq -j_iu_i.
\end{equation}

The total energy $\Pi_0[\Displacement,\phi]$ of a flexoelectric material is found by collecting all the internal and external energy densities as follows:

\begin{equation}\label{eq_Functional}
\Pi_0[\Displacement,\phi]=
\int_{\Omega}\Big(\mathcal{H}^\Omega[\Displacement,\phi]+\mathcal{W}^{\Omega}[\Displacement,\phi]\Big)\dd\Omega
+
\int_{\partial\Omega}\mathcal{W}^{\partial\Omega}_0[\Displacement,\phi]\dd\Gamma
+
\int_{C}\mathcal{W}^C_0[\Displacement,\phi]\dd\ds.
\end{equation}

The boundary of the domain $\partial\Omega$ can be split into several disjoint regions, corresponding to the different \emph{Dirichlet} and \emph{Neumann} boundaries. The external load is prescribed on the latter, whereas on the former its conjugate is prescribed.
For the mechanical loads, we have 
$\partial\Omega=\partial\Omega_u\cup\partial\Omega_t$
and
$\partial\Omega=\partial\Omega_v\cup\partial\Omega_r$.
The electrical part is also split into 
$\partial\Omega=\partial\Omega_\phi\cup\partial\Omega_w$.
The corresponding boundary conditions are
\begin{align}\label{strgr_classicalBC}
\Displacement - \DisplacementKnown &= \mathbf{0} \quad\text{on }{\partial\Omega_u},
&&&
\Traction(\Displacement,\phi) - \TractionKnown &= \mathbf{0} \quad\text{on }{\partial\Omega_t};
\\\label{strgr_nonlocalBC}
\partial^n(\Displacement) - \partialnDisplacementKnown &= \mathbf{0} \quad\text{on }{\partial\Omega_v},
&&&
\HighOrderTraction(\Displacement,\phi) - \HighOrderTractionKnown &= \mathbf{0} \quad\text{on }{\partial\Omega_r};
\\\label{elecBC}
\phi-\phiKnown &=0\quad\text{on }{\partial\Omega_\phi},
&&&
w(\Displacement,\phi)-\wKnown &=0\quad\text{on }{\partial\Omega_w};
\end{align}
where $\DisplacementKnown$, $\partialnDisplacementKnown$ and $\phiKnown$
are the prescribed
\emph{displacement}, \emph{normal derivative of the displacement} and \emph{electric potential} at the Dirichlet boundaries, and 
$\TractionKnown$, $\HighOrderTractionKnown$ and $\wKnown$
the prescribed \emph{traction}, \emph{double traction} and \emph{surface charge density} at the Neumann boundaries. The expressions $\Traction(\Displacement,\phi)$, $\HighOrderTraction(\Displacement,\phi)$ and $w(\Displacement,\phi)$ will be derived later as a result of the variational principle in \eq\eqref{eq_variationalPrinciple}.

The edges $C$ of $\partial\Omega$ are also split into $C=C_u\cup C_j$ corresponding to the Dirichlet and Neumann edge partitions, respectively. Here, $C_u$ is assumed to correspond to the curves within the classical Dirichlet boundary, namely $C_u=C\cap\overline{\partial\Omega_u}$, and $C_v=C\setminus C_u$. Edge boundary conditions are:
\begin{align}\label{strgr_edgeBC}
\Displacement - \DisplacementKnown &= \mathbf{0}\quad\text{on }{C_u},
&&&
\HighOrderJump(\Displacement,\phi) - \HighOrderJumpKnown &= \mathbf{0}\quad\text{on }{C_j},
\end{align}
where $\HighOrderJumpKnown$ is the prescribed \emph{force per unit length} at the Neumann edges, and the expression $\HighOrderJump(\Displacement,\phi)$ will be derived later from \eq\eqref{eq_variationalPrinciple}.
Many authors in the literature neglect the edge conditions in \eq\eqref{strgr_edgeBC} \cite{Aravas2011,Mao2014,Abdollahi2014,Abdollahi2015a}. It is important to note that dismissing them is equivalent to considering homogeneous Neumann edge conditions, which may not be true on $C_u$ (Dirichlet edges).
In this work, the edge conditions are kept in the formulation to ensure self-consistency and a well-defined boundary value problem.

The energy functional in \eq\eqref{eq_Functional} can be rewritten as follows, according to \eq(\ref{strgr_classicalBC}b)-(\ref{strgr_edgeBC}b):
\begin{equation}\label{eq_Functional2}
\Pi_0[\Displacement,\phi]=
\Pi^\Omega[\Displacement,\phi]
+
\Pi_0^\text{Dirichlet}[\Displacement,\phi]
+
\Pi^\text{Neumann}[\Displacement,\phi],
\end{equation}
where
\begin{equation}
\Pi^\Omega[\Displacement,\phi]=\int_{\Omega}\Big(\mathcal{H}^\Omega[\Displacement,\phi]+\mathcal{W}^{\Omega}[\Displacement,\phi]\Big)\dd\Omega,
\end{equation}
\begin{equation}\label{Dirichlet_0}
\Pi_0^\text{Dirichlet}[\Displacement,\phi]=
  \int_{\partial\Omega_u}-u_it_i(\Displacement,\phi)\dd\Gamma
  +
  \int_{\partial\Omega_v}-\partial^nu_ir_i(\Displacement,\phi)\dd\Gamma
  +
  \int_{\partial\Omega_\phi}\phi w(\Displacement,\phi)\dd\Gamma
  +
  \int_{C_u}-u_ij_i(\Displacement,\phi)\dd\ds
\end{equation}
and
\begin{equation}
\Pi^\text{Neumann}[\Displacement,\phi]=
\int_{\partial\Omega_t}-u_i\tractionKnown_i\dd\Gamma
+
\int_{\partial\Omega_r}-\partial^nu_i\highOrderTractionKnown_i\dd\Gamma
+
\int_{\partial\Omega_w}\phi\wKnown\dd\Gamma
+
\int_{C_j}-u_i\highOrderJumpKnown_i\dd\ds.
\end{equation}
The state variables 
$(\Displacement,\phi)\in\mathcal{U}_0\otimes\mathcal{P}_0$,
where
\begin{align}
\mathcal{U}_0 &\coloneqq\{\Displacement\in[\mathcal{H}^2(\Omega)]^3\text{ $|$ }
\Displacement-\DisplacementKnown=\mathbf{0}\text{ on }\partial\Omega_u,
\Displacement-\DisplacementKnown=\mathbf{0}\text{ on }C_u
\text{ and }
\partial^n\Displacement-\partialnDisplacementKnown=\mathbf{0}\text{ on }\partial\Omega_v\},
\\
\mathcal{P}_0 &\coloneqq\{\phi\in\mathcal{H}^1(\Omega)\text{ $|$ }
\phi-\phiKnown=0\text{ on }\partial\Omega_\phi\};
\end{align}
fulfilling Dirichlet boundary conditions in \eq (\ref{strgr_classicalBC}a)-(\ref{strgr_edgeBC}a).

The equilibrium states $(\Displacement^*,\phi^*)$ of the body correspond to the following variational principle:
\begin{equation}\label{eq_variationalPrinciple}
(\Displacement^\text*,\phi^\text*)=\arg\min_{\Displacement\in\mathcal{U}_0}\max_{\phi\in\mathcal{P}_0}\Pi_0[\Displacement,\phi].
\end{equation}

The Euler-Lagrange equations associated with the variational principle in \eq\eqref{eq_variationalPrinciple} and the expressions $\Traction(\Displacement,\phi)$, $\HighOrderTraction(\Displacement,\phi)$, $w(\Displacement,\phi)$ and $\HighOrderJump(\Displacement,\phi)$ from the Neumann boundary conditions in \eq (\ref{strgr_classicalBC}b)-(\ref{strgr_edgeBC}b) are found by enforcing
%
\begin{subequations}\begin{align}
\var{\Pi_0}=\var[\Displacement]{\Pi_0}+\var[\phi]{\Pi_0}=0
;\label{eq_1var}
\\
\vvar[\Displacement]{\Pi_0}>0,\quad
\vvar[\phi]{\Pi_0}<0
,\label{eq_2var}
\end{align}\end{subequations}
%
for all admissible variations
$\delta\Displacement\in\mathcal{U}_0$ and $\delta\phi\in\mathcal{P}_0$. 
The full derivation can be found in \cite{Liu2014}, and the resulting equations are given next \cite{Liu2014,Mao2014,Abdollahi2014, Abdollahi2015a, Abdollahi2015b}:
\begin{equation}\label{eq_EulerLagrange}
\begin{cases}
\left(\cauchyStress_{ij}(\Displacement,\phi)-\hyperStress_{ijk,k}(\Displacement,\phi)\right)_{,j}+b_i=0_i &\text{in }\Omega,\\
\hfill\electricDisp_{l,l}(\Displacement,\phi)-q=0\hphantom{{}_i} & \text{in }\Omega;
\end{cases}
\end{equation}
and
\begin{subnumcases}{\label{eq_FlexoForces}}
t_i(\Displacement,\phi) \coloneqq \left(\cauchyStress_{ij}(\Displacement,\phi)-\hyperStress_{ijk,k}(\Displacement,\phi)-\surfaceGradient_{k}\hyperStress_{ikj}(\Displacement,\phi)\right)n_j+\hyperStress_{ijk}(\Displacement,\phi)\curvatureProjector_{jk}
& on $\partial\Omega$ \label{eq_Traction},\\
r_i(\Displacement,\phi) \coloneqq \hyperStress_{ijk}(\Displacement,\phi)n_jn_k
& on $\partial\Omega$, \\
w(\Displacement,\phi) \coloneqq -\electricDisp_l(\Displacement,\phi)n_l
& on $\partial\Omega$, \\
j_i(\Displacement,\phi) \coloneqq \jump{\hyperStress_{ijk}(\Displacement,\phi)m_jn_k}
& on $C$.
\end{subnumcases}

Note that the traction $\Traction(\Displacement,\phi)$ in \eq\eqref{eq_Traction} is an alternative expression to the one in \cite{Mindlin1964}, whose derivation can be found in \ref{sec_app01}.

In \eq\eqref{eq_EulerLagrange} and \eqref{eq_FlexoForces}, the \emph{stress} $\CauchyStress(\Displacement,\phi)$, the \emph{double stress} $\HyperStress(\Displacement,\phi)$ and the \emph{electric displacement} $\ElectricDisp(\Displacement,\phi)$ are defined as the conjugates to the strain $\Strain(\Displacement)$, the strain gradient $\gradient\Strain(\Displacement)$ and the electric field $\E(\phi)$, respectively, as follows:
\begin{subequations}\label{elec_tensors}\begin{align}
\cauchyStress_{ij}(\Displacement,\phi)=\cauchyStress_{ji}(\Displacement,\phi)
&\coloneqq
\left.\frac{\partial \mathcal{H}^\Omega[\Strain,\gradient\Strain,\E]}{\partial\strain_{ij}}\right|_{\substack{\Strain=\Strain(\Displacement)\\\E=\E(\phi)}}
=\elast_{ijkl}\strain_{kl}(\Displacement)-\piezo_{lij}E_{l}(\phi);
\\
\hyperStress_{ijk}(\Displacement,\phi)=\hyperStress_{jik}(\Displacement,\phi)
&\coloneqq
\left.\frac{\partial\mathcal{H}^\Omega[\Strain,\gradient\Strain,\E]}{\partial\strain_{ij,k}}\right|_{\substack{\gradient\Strain=\gradient\Strain(\Displacement)\\\E=\E(\phi)}}
=\strGr_{ijklmn}\strain_{lm,n}(\Displacement)-\flexo_{lijk}E_{l}(\phi);
\\
\electricDisp_l(\Displacement,\phi)
&\coloneqq
\left.-\frac{\partial\mathcal{H}^\Omega[\Strain,\gradient\Strain,\E]}{\partial E_{l}}\right|_{\substack{\Strain=\Strain(\Displacement)\\\E=\E(\phi)\\\gradient\Strain=\gradient\Strain(\Displacement)}}
=\dielec_{lm}E_{m}(\phi)+\piezo_{lij}\strain_{ij}(\Displacement)+\flexo_{lijk}\strain_{ij,k}(\Displacement).
\end{align}\end{subequations}

The positivity and negativity conditions on the second variations in \eq\eqref{eq_2var} lead to the following restrictions on the material tensors:
\begin{align}\label{restrictions}
\dielec_{ii}>0, \qquad
\elast_{ijij}>0, \qquad
\strGr_{ijkijk}\geq0
%, &&
%\piezo_{lij}\piezo_{lij}<\elast_{ijij}\dielec_{ll}, &&
%\flexo_{lijk}\flexo_{lijk}<\strGr_{ijkijk}\dielec_{ll}
; &&
&& \quad i,j,k
%,l
&=1,\dots,n_d,
\end{align}
being $n_d$ the number of spatial dimensions. 

\begin{remark}
	This formulation corresponds to the 3D case. It also holds for 2D with the following considerations:
	\vspace{-0.5em}\begin{itemize}\setlength\itemsep{-0.3em}
		\item The vectors $\n$ and $\m$ defined on the \emph{curve} $\partial\Omega_f$ refer to the outward unit normal and tangent vectors, respectively (see \fig\ref{fig_3_1}).
		\item The edges $C$ in \eq\eqref{eq_Functional} correspond to \emph{corners} of $\partial\Omega$, and therefore have dimension 0. As a consequence, their contribution to the external work $\int_{C}\HighOrderJump\delta\Displacement\dd\ds$ is $\sum_C\HighOrderJump\delta\Displacement$ in \eq\eqref{eq_Functional} and subsequent terms.
	\end{itemize}
\end{remark}
\begin{figure}[t]\centering
	%	\begin{subfigure}[t]{.17\textwidth}\centering
	%		\captionof{figure}{}
	%		\includegraphics[scale=0.17]{Images/Sec_02/1c2.pdf}
	%		\vfill\label{fig_2_1_1}
	%	\end{subfigure}%
	\begin{subfigure}[t]{.3\textwidth}\centering
		\captionof{figure}{}\vspace{-0.5em}
		\includegraphics[scale=0.17]{Images/Sec_02/5c_.pdf}
		\vfill\label{fig_3_1_2}
	\end{subfigure}%
	\begin{subfigure}[t]{.3\textwidth}\centering
		\captionof{figure}{}\vspace{-0.5em}
		\includegraphics[scale=0.17]{Images/Sec_02/6c_.pdf}
		\vfill\label{fig_3_1_3}
	\end{subfigure}%
	\begin{subfigure}[t]{.3\textwidth}\centering
		\captionof{figure}{}\vspace{-0.5em}
		\includegraphics[scale=0.17]{Images/Sec_02/7c_.pdf}
		\vfill\label{fig_3_1_4}
	\end{subfigure}
	\caption{Sketch of the geometry of $\Omega\in\mathbb{R}^2$.
		\emph{a)} $\Omega$ and the boundary $\partial\Omega$ subdivided in several smooth portions $\partial\Omega_f$, \eg $\partial\Omega_i$ and $\partial\Omega_j$ with their corresponding normal vectors $\n^i$ and $\n^j$. The intersection between $\partial\Omega_i$ and $\partial\Omega_j$ is the corner $C^{ij}$. \emph{b)} Detail of $\partial\Omega_i$, with the pair $\{\m^i,\n^i$ defined on $C^{ij}$, and \emph{c)} detail of $\partial\Omega_j$, with the pair $\{\m^j,\n^j\}$ defined on $C^{ij}$.}
	\label{fig_3_1}
\end{figure}
%%%%%
\subsection{Variational formulation within an unfitted framework: The Nitsche's method}
%%%%%
The admissible space $\mathcal{U}_0\otimes\mathcal{P}_0$ of the state variables $(\Displacement,\phi)$ is constrained on the Dirichlet boundaries, and therefore is not suitable for an unfitted formulation. In order to overcome this requirement, an alternative energy functional $\Pi[\Displacement,\phi]$ is proposed following Nitsche's approach \cite{Nitsche1971}:
\begin{equation}\label{eq_Functionalimm}
\Pi[\Displacement,\phi]=
\Pi^\Omega[\Displacement,\phi]
+
\Pi^\text{Dirichlet}[\Displacement,\phi]
+
\Pi^\text{Neumann}[\Displacement,\phi],
\end{equation} 
where $\Pi^\text{Dirichlet}[\Displacement,\phi]$ acts on the Dirichlet boundaries instead of $\Pi_0^\text{Dirichlet}[\Displacement,\phi]$, and incorporates Dirichlet boundary conditions in \eq(\ref{strgr_classicalBC}a)-(\ref{strgr_edgeBC}a) weakly as follows:
\begin{multline}\label{Dirichlet}
\Pi^\text{Dirichlet}[\Displacement,\phi]=
\int_{\partial\Omega_u}\left(\frac{1}{2}\beta_u\Big(u_i-\displacementKnown_i\Big)^2-\Big(u_i-\displacementKnown_i\Big)t_i(\Displacement,\phi)\right)\dd\Gamma
+
\int_{\partial\Omega_v}\left(\frac{1}{2}\beta_v\Big(\partial^nu_i-\partialndisplacementKnown_i\Big)^2-\Big(\partial^nu_i-\partialndisplacementKnown_i\Big)r_i(\Displacement,\phi)\right)\dd\Gamma
+{}\\{}+
\int_{\partial\Omega_\phi}\left(-\frac{1}{2}\beta_\phi\Big(\phi-\phiKnown\Big)^2+\Big(\phi-\phiKnown\Big) w(\Displacement,\phi)\right)\dd\Gamma
+
\int_{C_u}\left(\frac{1}{2}\beta_{C_u}\Big(u_i-\displacementKnown_i\Big)^2-\Big(u_i-\displacementKnown_i\Big)j_i(\Displacement,\phi)\right)\dd\ds,
\end{multline}
with the numerical parameters $\beta_u,\beta_v,\beta_{C_u},\beta_\phi\in\mathds{R}^+$.

Comparing \eq\eqref{Dirichlet} against \eq\eqref{Dirichlet_0}, one can readily see that the expressions $\Traction(\Displacement,\phi)$, $\HighOrderTraction(\Displacement,\phi)$, $w(\Displacement,\phi)$ and $\HighOrderJump(\Displacement,\phi)$ are now conjugate to the Dirichlet boundary conditions.
The (positive or negative) penalty terms inserted in each boundary integral are quadratic in the Dirichlet boundary conditions, and its only purpose is to ensure equilibrium states $(\Displacement^*,\phi^*)$ being, respectively, actual minima and maxima of the energy functional with respect to $\Displacement$ and $\phi$.

The variational principle associated to $\Pi[\Displacement,\phi]$ for the equilibrium states $(\Displacement^*,\phi^*)$ of the body is stated next:
\begin{equation}\label{variationalPrinciple}
(\Displacement^\text*,\phi^\text*)=\arg\min_{\Displacement\in\mathcal{U}}\max_{\phi\in\mathcal{P}}\Pi[\Displacement,\phi],
\end{equation}
where $\mathcal{P}\coloneqq\mathcal{H}^1(\Omega)$, and $\mathcal{U}$ is the space of functions belonging to $\big[\mathcal{H}^2(\Omega)\big]^3$ with $\mathcal{L}^2$-integrable third derivatives on the boundary $\partial\Omega_u$, to account for the integrals involving $\Traction(\Displacement,\phi)$ in \eq\eqref{eq_Traction}.
The variational principle in \eq\eqref{variationalPrinciple} leads to the same Euler-Lagrange equations in \eq\eqref{eq_EulerLagrange} and definitions of $\Traction(\Displacement,\phi)$, $\HighOrderTraction(\Displacement,\phi)$, $w(\Displacement,\phi)$ and $\HighOrderJump(\Displacement,\phi)$ in \eq\eqref{eq_FlexoForces} as the constrained variational principle in \eq\eqref{eq_variationalPrinciple}.

The penalty parameters $\beta_u,\beta_v,\beta_{C_u},\beta_\phi$ in \eq\eqref{Dirichlet} have to be chosen large enough, but too large values would lead to ill-conditioning problems when finding the equilibrium states $(\Displacement^*,\phi^*)$ numerically.
The derivation of stability lower bounds of the penalty parameters can be found in \ref{sec_app02}. However, moderate values of the penalty parameters are enough to ensure convergence and enforce boundary conditions properly \cite{Fernandez2004,Schillinger2016}.

%%%%%
\subsection{Weak form of the boundary value problem}
%%%%%
The weak form of the unfitted variational formulation is presented next. 
Vanishing of the first variation of \eq\eqref{eq_Functionalimm} yields
\begin{equation}\label{firstvariation}
0=\var{\Pi}[\Displacement,\phi;\delta\Displacement,\delta\phi]=
\var{\Pi^\Omega}[\Displacement,\phi;\delta\Displacement,\delta\phi]
+
\var{\Pi^\text{Dirichlet}}[\Displacement,\phi;\delta\Displacement,\delta\phi]
+
\var{\Pi^\text{Neumann}}[\delta\Displacement,\delta\phi],
\quad
\forall(\delta\Displacement,\delta\phi)\in\mathcal{U}\otimes\mathcal{P};
\end{equation}
where
\begin{subequations}\begin{align}
\var{\Pi^\Omega}[\Displacement,\phi;\delta\Displacement,\delta\phi]&=
\int_{\Omega}\Big(\cauchyStress_{ij}(\Displacement,\phi)\strain_{ij}(\delta\Displacement)+\hyperStress_{ijk}(\Displacement,\phi)\strain_{ij,k}(\delta\Displacement)-\electricDisp_l(\Displacement,\phi)E_l(\delta\phi)-b_i\delta u_{i}+q\delta \phi\Big)\dd\Omega,
\\
\var{\Pi^\text{Dirichlet}}[\Displacement,\phi;\delta\Displacement,\delta\phi]&=
\int_{\partial\Omega_u}\Big(\beta_u\Big(u_i-\displacementKnown_i\Big)\delta u_i
-t_i(\Displacement,\phi)\delta u_i
-\Big(u_i-\displacementKnown_i\Big)t_i(\delta\Displacement,\delta\phi)\Big)\dd\Gamma
+{}\nonumber\\&{}+
\int_{\partial\Omega_v}\Big(\beta_v\Big(\partial^nu_i-\partialndisplacementKnown_i\Big)\partial^n\delta u_i
-r_i(\Displacement,\phi)\partial^n\delta u_i
-\Big(\partial^nu_i-\partialndisplacementKnown_i\Big)r_i(\delta\Displacement,\delta\phi)\Big)\dd\Gamma
+{}\nonumber\\&{}+
\int_{\partial\Omega_\phi}\Big(-\beta_\phi\Big(\phi-\phiKnown\Big)\delta\phi
+w(\Displacement,\phi)\delta\phi 
+\Big(\phi-\phiKnown\Big) w(\delta\Displacement,\delta\phi)\Big)\dd\Gamma
+{}\nonumber\\&{}+
\int_{C_u}\Big(\beta_{C_u}\Big(u_i-\displacementKnown_i\Big)\delta u_i
-j_i(\Displacement,\phi)\delta u_i 
-\Big(u_i-\displacementKnown_i\Big)j_i(\delta\Displacement,\delta\phi)\Big)\dd\ds,
\\
\var{\Pi^\text{Neumann}}[\delta\Displacement,\delta\phi]&=
\int_{\partial\Omega_t}-\tractionKnown_i\delta u_i\dd\Gamma
+
\int_{\partial\Omega_r}-\highOrderTractionKnown_i\partial^n\delta u_i\dd\Gamma
+
\int_{\partial\Omega_w}\wKnown\delta\phi\dd\Gamma
+
\int_{C_j}-\highOrderJumpKnown\delta u_i\dd\ds;
\end{align}\end{subequations}
being $\delta\Displacement\in\mathcal{U}$ and $\delta\phi\in\mathcal{P}$ admissible variations of $\Displacement$ and $\phi$, respectively.

The functionals $\var{\Pi^\Omega}$ and $\var{\Pi^\text{Dirichlet}}$ are conveniently rearranged as $\var{\Pi^\Omega}[\Displacement,\phi;\delta\Displacement,\delta\phi]=\var{\Pi^\Omega_\mathscr{B}}[\Displacement,\phi;\delta\Displacement,\delta\phi]-\var{\Pi^\Omega_\mathscr{L}}[\delta\Displacement,\delta\phi]$ and $\var{\Pi^\text{Dirichlet}}[\Displacement,\phi;\delta\Displacement,\delta\phi]=\var{\Pi^\text{Dirichlet}_\mathscr{B}}[\Displacement,\phi;\delta\Displacement,\delta\phi]-\var{\Pi^\text{Dirichlet}_\mathscr{L}}[\delta\Displacement,\delta\phi]$, with
\begin{subequations}\begin{align}
\var{\Pi^\Omega_\mathscr{B}}[\Displacement,\phi;\delta\Displacement,\delta\phi]&\coloneqq
\int_{\Omega}\Big(\cauchyStress_{ij}(\Displacement,\phi)\strain_{ij}(\delta\Displacement)+\hyperStress_{ijk}(\Displacement,\phi)\strain_{ij,k}(\delta\Displacement)-\electricDisp_l(\Displacement,\phi)E_l(\delta\phi)\Big)\dd\Omega,
\\
\var{\Pi^\Omega_\mathscr{L}}[\delta\Displacement,\delta\phi]&\coloneqq
\int_{\Omega}\Big(b_i\delta u_{i}-q\delta \phi\Big)\dd\Omega,
\\
\var{\Pi^\text{Dirichlet}_\mathscr{B}}[\Displacement,\phi;\delta\Displacement,\delta\phi]&\coloneqq
\int_{\partial\Omega_u}\Big(\Big(\beta_uu_i-t_i(\Displacement,\phi)\Big)\delta u_i
-u_it_i(\delta\Displacement,\delta\phi)\Big)\dd\Gamma
+{}\nonumber\\&{}+
\int_{\partial\Omega_v}\Big(\Big(\beta_v\partial^nu_i-r_i(\Displacement,\phi)\Big)\partial^n\delta u_i
-\partial^nu_ir_i(\delta\Displacement,\delta\phi)\Big)\dd\Gamma
+{}\nonumber\\&{}+
\int_{\partial\Omega_\phi}\Big(\Big(-\beta_\phi\phi+w(\Displacement,\phi)\Big)\delta\phi
+\phi w(\delta\Displacement,\delta\phi)\Big)\dd\Gamma
+{}\nonumber\\&{}+
\int_{C_u}\Big(\Big(\beta_{C_u}u_i-j_i(\Displacement,\phi)\Big)\delta u_i
-u_ij_i(\delta\Displacement,\delta\phi)\Big)\dd\ds,
\\
\var{\Pi^\text{Dirichlet}_\mathscr{L}}[\delta\Displacement,\delta\phi]&\coloneqq
\int_{\partial\Omega_u}\displacementKnown_i\Big(\beta_u\delta u_i-t_i(\delta\Displacement,\delta\phi)\Big)\dd\Gamma
+
\int_{\partial\Omega_v}\partialndisplacementKnown_i\Big(\beta_v\partial^n\delta u_i-r_i(\delta\Displacement,\delta\phi)\Big)\dd\Gamma
+{}\nonumber\\&{}+
\int_{\partial\Omega_\phi}\phiKnown\Big(-\beta_\phi\delta\phi+w(\delta\Displacement,\delta\phi)\Big)\dd\Gamma
+
\int_{C_u}\displacementKnown_i\Big(\beta_{C_u}\delta u_i-j_i(\delta\Displacement,\delta\phi)\Big)\dd\ds,
\end{align}\end{subequations}

The weak form of the unfitted formulation for flexoelectricity reads:
\begin{equation}\label{eq_FlexWeakSymmNitsche}
\emph{Find $(\Displacement,\phi)\in\mathcal{U}\otimes\mathcal{P}$ such that $\forall(\delta\Displacement,\delta\phi)\in\mathcal{U}\otimes\mathcal{P}:$}\quad
\mathscr{B}[\{\Displacement,\phi\},\{\delta\Displacement,\delta\phi\}]
=
\mathscr{L}[\{\delta\Displacement,\delta\phi\}]
;
\end{equation}
where
\begin{subequations}\begin{align}
\mathscr{B}[\{\Displacement,\phi\},\{\delta\Displacement,\delta\phi\}]&\coloneqq
\var{\Pi^\Omega_\mathscr{B}}[\Displacement,\phi;\delta\Displacement,\delta\phi]+\var{\Pi^\text{Dirichlet}_\mathscr{B}}[\Displacement,\phi;\delta\Displacement,\delta\phi],
\label{bil}\\
\mathscr{L}[\{\delta\Displacement,\delta\phi\}]&\coloneqq
\var{\Pi^\Omega_\mathscr{L}}[\delta\Displacement,\delta\phi]+\var{\Pi^\text{Dirichlet}_\mathscr{L}}[\delta\Displacement,\delta\phi]+\var{\Pi^\text{Neumann}}[\delta\Displacement,\delta\phi].
\end{align}\end{subequations}

%%%%%%%
\subsection{Formulation including sensing electrodes}\label{sec_03bis}
%%%%%%%
In electromechanics, conducting electrodes are frequently attached to the surface of the devices to enable either \emph{actuation} or \emph{sensing}. Actuators induce a deformation due to a prescribed electric potential, whereas sensors infer the deformation state by the measured change in the electric potential.
In both cases, as the electrodes are made of conducting material, the electric potential in the electrode is uniform.
The electrical Dirichlet boundary condition in \eq\eqref{elecBC} corresponds to actuating electrodes where the uniform electric potential is prescribed. In the case of sensing electrodes, the uniform electric potential is unknown and thus requires a special treatment as described next.

Let us consider a partition of the boundary distinguishing actuating and sensing electrodes, \ie
\begin{equation}
\partial\Omega=\partial\Omega_{\phi}\cup\partial\Omega_{\Phi}\cup\partial\Omega_{w},
\end{equation}
where $\partial\Omega_{\phi}$ and $\partial\Omega_{\Phi}$ correspond, respectively, to actuating and sensing electrodes on the boundary, respectively, and $\partial\Omega_{w}$ to the electrical Neumann boundary. The sensing boundary $\partial\Omega_{\Phi}$ is conformed by $N_\text{sensing}$ electrodes, namely
$
\partial\Omega_{\Phi}=\bigcup_{i=1}^{N_\text{sensing}}{\partial\Omega_{\Phi}}^i.
$

The electric potential $\phi$ on sensing electrodes is constant, but unknown. Thus, at each electrode ${\partial\Omega_{\Phi}}^i$ a new state variable ${\Phi}^i\in\mathbb{R}$ is introduced, which is a scalar denoting the unknown constant value of the electric potential. In other words,
\begin{equation}\label{eq_sensor1}
\phi-\Phi^i=0 \quad\text{on }{{\partial\Omega_{\Phi}}^i},\quad\forall i=1,\dots,N_\text{sensing}.
\end{equation}
Boundary conditions in \eq\eqref{eq_sensor1} are weakly enforced by adding to the energy potential $\Pi[\Displacement,\phi]$ in \eq\eqref{eq_Functionalimm} the work $\Pi^\text{Sensing}_i[\Displacement,\phi,\Phi^i]$ of each sensing electrode:
\begin{equation}\label{Sensor}
\Pi^\text{Sensing}_i[\Displacement,\phi,\Phi^i]=
\int_{\partial\Omega_\Phi^i}\Big(\phi-\Phi^i\Big) w(\Displacement,\phi)\dd\Gamma,
\end{equation}
and the associated variational principle for the equilibrium states $(\Displacement^*,\phi^*,\Phi^{1*},\dots,\Phi^{{N_\text{sensing}}*})$ of the body is
\begin{equation}\label{variationalPrincipleSensor}
(\Displacement^*,\phi^*,\Phi^{1*},\dots,\Phi^{{N_\text{sensing}}*})=\arg\min_{\Displacement\in\mathcal{U}}\max_{\phi\in\mathcal{P}}\min_{\Phi^1\in\mathbb{R}}\dots\min_{\Phi^{N_\text{sensing}}\in\mathbb{R}}\left(\Pi[\Displacement,\phi]+\sum_{i=1}^{N_\text{sensing}}\Pi^\text{Sensing}_i[\Displacement,\phi,\Phi^i]\right).
\end{equation}
Equation \eqref{Sensor} has a similar form to the Nitsche terms $\Pi^\text{Dirichlet}[\Displacement,\phi]$ in \eq\eqref{Dirichlet}, but the penalty term quadratic in \eq\eqref{eq_sensor1} is omitted here since $\phi$ and $\Phi^i$ are to be maximized and minimized, respectively. Vanishing of the first variation of the energy functional in \eq\eqref{variationalPrincipleSensor} yields
\begin{equation}
0=\var{\Pi}[\Displacement,\phi;\delta\Displacement,\delta\phi]
+\sum_{i=1}^{N_\text{sensing}}\var{\Pi^\text{Sensing}_i}[\Displacement,\phi,\Phi^i;\delta\Displacement,\delta\phi,\delta\Phi^i],
\end{equation}
where
\begin{equation}
\var{\Pi^\text{Sensing}_i}[\Displacement,\phi,\Phi^i;\delta\Displacement,\delta\phi,\delta\Phi^i]\coloneqq
\int_{\partial\Omega_\Phi^i}\Big(\phi-\Phi^i\Big) w(\delta\Displacement,\delta\phi)\dd\Gamma+
\int_{\partial\Omega_\Phi^i}w(\Displacement,\phi)\Big(\delta\phi-\delta\Phi^i\Big)\dd\Gamma,
\end{equation}
being $\delta\Phi^i\in\mathbb{R}$ admissible variations of each $\Phi^i$.
Finally, the weak form of the unfitted formulation for flexoelectricity accounting for sensing electrodes reads:
\begin{multline}\label{eq_FlexWeakSymmNitscheSensor}
\emph{Find $(\Displacement,\phi,\Phi^1,...,\Phi^{N_\text{sensing}})\in\mathcal{U}\otimes\mathcal{P}\otimes\mathbb{R}^{N_\text{sensing}}$ such that $\forall(\delta\Displacement,\delta\phi,\delta\Phi^1,...,\delta\Phi^{N_\text{sensing}})\in\mathcal{U}\otimes\mathcal{P}\otimes\mathbb{R}^{N_\text{sensing}}:$}\\
\mathscr{B}[\{\Displacement,\phi\},\{\delta\Displacement,\delta\phi\}]
+
\sum_{i=1}^{N_\text{sensing}}\var{\Pi^\text{Sensing}_i}[\Displacement,\phi,\Phi^i;\delta\Displacement,\delta\phi,\delta\Phi^i]
=
\mathscr{L}[\{\delta\Displacement,\delta\phi\}]
.\end{multline}
